Inference procedures in sequential trial emulation with survival outcomes: comparing confidence intervals based on the sandwich variance estimator, bootstrap and jackknife

Sequential trial emulation (STE) is an approach to estimating causal treatment effects by emulating a sequence of target trials from observational data. In STE, inverse probability weighting is commonly utilised to address time-varying confounding and/or dependent censoring. Then structural models for potential outcomes are applied to the weighted data to estimate treatment effects. For inference, the simple sandwich variance estimator is popular but conservative, while nonparametric bootstrap is computationally expensive, and a more efficient alternative, linearised estimating function (LEF) bootstrap, has not been adapted to STE. We evaluated the performance of various methods for constructing confidence intervals (CIs) of marginal risk differences in STE with survival outcomes by comparing the coverage of CIs based on nonparametric/LEF bootstrap, jackknife, and the sandwich variance estimator through simulations. LEF bootstrap CIs demonstrated the best coverage with small/moderate sample sizes, low event rates and low treatment prevalence, which were the motivating scenarios for STE. They were less affected by treatment group imbalance and faster to compute than nonparametric bootstrap CIs. With large sample sizes and medium/high event rates, the sandwich-variance-estimator-based CIs had the best coverage and were the fastest to compute. These findings offer guidance in constructing CIs in causal survival analysis using STE.

==> results_before_amend_2405.tex <==
\subsubsection{CI coverage}\label{CIresults}
Figure~\ref{fig:coverage_low} shows the empirical coverage rates of the CIs when the event rate was low; see Figures 2 and 3 of the Supplementary Materials for results with medium and high event rates.
Figures 4, 5 and 6 of the Supplementary Materials show the bias-eliminated empirical coverage rates, which are slightly different from empirical coverage results for scenarios with non-negligible empirical biases. However, these differences are negligible. 

\begin{sidewaysfigure}[h!]
 \centering
 \includegraphics[width = \textwidth]{pivot_coverage_low.jpeg}
 \caption{Coverage of the CIs in the scenarios with low event rates. Bootstrap: CIs constructed by nonparametric bootstrap; LEF both: CIs constructed by applying Approach 2 of LEF bootstrap; LEF outcome: CIs constructed by applying Approach 1 of LEF bootstrap; Jackknife Wald: CIs constructed by applying Approach 1 of jackknife resampling; jackknife MVN: CIs constructed by applying Approach 2 of jackknife resampling; Sandwich: CIs based on the sandwich variance estimator. Note that the results for applying Approaches 1 and 2 of LEF bootstrap were very similar so that the purple and green lines overlapped.}
 \label{fig:coverage_low}
\end{sidewaysfigure}


\emph{\textbf{Impact of trial follow-up visits}.} \hl{ At earlier visits ($k\le 2$), } there was a general pattern of coverage getting closer to the nominal 95\% level for all CI methods as the sample size increases, which was not surprising given that all the methods rely on asymptotic approximations. There was also a general trend of coverage being lower at later visits. This was likely because there were very few events occurred after trial visit $2$ in most scenarios, even those with large sample sizes ($n = 5000$) (see Table 3 of Supplementary Materials for an example).

\emph{\textbf{Impact of treatment prevalence and sample size}.} In scenarios with low/medium treatment prevalence ($\alpha_a = -1, 0$) and small/medium sample sizes ($n = 200,1000$), nonparametric bootstrap CIs generally %consistently
exhibited lower coverage compared to LEF bootstrap CIs. For large samples ($n = 5000$), all bootstrap methods performed similarly. This discrepancy may be due to the instability of parameter estimation in nonparametric bootstrap  for scenarios with small/medium sample sizes and low event rates, which was reduced in LEF bootstrap by design. Similar findings for nonparametric bootstrap CIs were also observed by Austin (2022) \cite{austin_bootstrap_2022}.   

Sandwich CIs showed the worst coverage with small sample sizes ($n = 200$) and low  treatment prevalence ($\alpha_a = -1$), never achieving the nominal 95\% level and sometimes falling as low as 70\%. This poor performance might be explained by 1) the sandwich variance estimation suffering from small-sample bias 2) the large number of construction failures for the sandwich variance estimator when $n=200$  (see Section 5.8 of the Supplementary Materials for more details). The  low coverage  of  Sandwich CIs may have been to some extent mitigated by the positive asymptotic bias of the sandwich variance estimator \cite{austin_variance_2016}. With medium treatment prevalence  and small sample sizes, Sandwich CIs performed similarly as nonparametric bootstrap CIs, both worse than LEF bootstrap CIs. 


For low treatment prevalence ($\alpha_a = -1$) and small sample size ($n = 200$) scenarios,  jackknife Wald CIs were close to the nominal 95\% coverage at all visits, however, this coverage decreased as the treatment prevalence increased ($\alpha_a= 0,1$). Similar patterns were observed for  jackknife MVN CIs, although with medium treatment prevalence they performed better than jackknife Wald CIs.  

High treatment prevalence ($\alpha_a = 1$) resulted in considerable disparities in CI coverage across the methods. Coverage decayed considerably at later visits across most methods, with nominal coverage rarely achieved at post-baseline visit ($k \geq 1$). Nonparametric bootstrap  CIs had the most prominent decrease of coverage over time, while Sandwich CIs, though not reaching nominal coverage, performed better than nonparametric bootstrap CIs. For small sample sizes, both jackknife-based CIs exhibited very poor coverage that slightly increased at later visits. With small and medium sample sizes, LEF bootstrap CIs performed similarly as Sandwich CIs and much better than nonparametric bootstrap  CIs.
With large sample sizes, Sandwich CIs approached nominal coverage at earlier visits but remained suboptimal (around 70\% coverage) at later visits, while all bootstrap methods lagged by about 10\%. This was the only simulation scenario in Figure~\ref{fig:coverage_low} where the coverage of Sandwich CIs surpassed that of LEF bootstrap CIs. This reversal in performance highlights the impact of sample size on the performance of the CI  methods. 
With small sample sizes and low event rates, the sandwich variance estimator exhibited finite-sample bias and encountered many construction failures, which resulted in poorer CI coverage than  LEF bootstrap CIs. With larger sample sizes, these issues of the sandwich variance estimator diminished. On the other hand,  high treatment prevalence and low event rates exacerbated the treatment imbalances and data sparsity at later visits as seen in the data tabulation examples in Tables 1, 2 and 3 of the Supplementary Materials, which greatly affected the performance of the LEF bootstrap (even if the sample sizes were large) and jackknife methods. 

\emph{\textbf{Impact of confounding strength and outcome event rates}.} We observed minimal impact of confounding strength on CI coverage, perhaps because the values of $\alpha_c$ had relatively small influences on the MRD estimation given the impact of treatment prevalence.

Increasing outcome event rates improved the CI coverage for all methods, as shown in Figures 2 and 3 of the Supplementary Materials. %It was previously noted that higher event rates reduce absolute bias in the MRD estimation analysis, likely due to increased event information. 
 The impact of treatment prevalence on jackknife Wald CIs coverage was reduced when increasing the outcome event rates, as jackknife Wald CIs were close to nominal coverage rates in low and medium treatment prevalence scenarios ($\alpha_a = -1,0$) with small sample sizes ($n = 200$) and high event rate. Jackknife MVN CIs were exhibiting slight over-coverage in such scenarios, while they had the best coverage in high treatment prevalence and high event rate scenarios.
 
With medium event rates and small sample sizes, Sandwich CIs and non-parametric bootstrap CIs had better coverage than when the event rate was low, but still performed worse than LEF bootstrap CIs.The sandwich variance estimator was likely less biased and its construction failures were much less frequent under higher event rates. Likewise, bootstrap samples with very few or no events would be less common. However, the instability of parameter estimation in nonparametric bootstrap still existed, which led to worse coverage of nonparametric bootstrap CIs than LEF bootstrap CIs.  

With high event rates and small sample sizes, the performance of Sandwich CIs was further improved from medium event rate scenarios, but similarly as the LEF bootstrap CIs. Similar to low/medium outcome rate scenarios, LEF bootstrap CIs performed better than non-parametric bootstrap CIs in high outcome rate and small sample size scenarios. 
With high event rates and medium/large sample sizes, all methods performed similarly. 


\subsubsection{Empirical bias}

Figure~\ref{bias} presented the empirical biases of the MRD estimates.
Minimal biases were observed at earlier visits ($k < 2$).
But with small sample sizes ($n = 200$), the MRD estimates at later visits ($k >3 $) exhibited non-negligible bias, especially when the treatment prevalence was low ($\alpha_a= -1$) or high ($\alpha_a= 1$) and confounding was the strongest ($\alpha_c=0.9$).
This bias approached zero as sample sizes increased. The increasing bias at later visits coincided with the deterioration in CI coverage that we observed across all data scenarios at later visits (reason (i) of  under-coverage according to Morris et al. \cite{morris_using_2019}), which could be due to the increasing data sparsity and treatment imbalances at later visits. 
\begin{sidewaysfigure}[h!]
 \centering
 \includegraphics[width = \textwidth]{bias_all.jpeg}
 \caption{Empirical biases of the MRD estimates in various simulation scenarios.}
 \label{bias}
\end{sidewaysfigure}
\hl{The biases under small sample sizes and low/medium event rate showed different directions across the scenarios of treatment prevalence and confounding strength. In scenarios with high treatment prevalence, the biases were negative, which indicated treatment effect overestimation (as the MRD was negative and underestimated) at later visits. We can see from Figures} \ref{bias-0} and \ref{bias-1} \hl{showing the empirical bias of the survival probability estimates in }\eqref{mrd formula counterfactuals} \hl{that MRD underestimation was due to underestimation of  survival probability in the never-treated. Conversely, the MRD estimation bias under low treatment prevalence was positive indicating overestimation of the MRD, which was caused by underestimation of the  survival probability in the always-treated as seen in Figure }\ref{bias-1}. \hl{Increasing the confounding strength also tended to increase absolute bias.}

 \hl{The different directions and magnitudes of  biases were likely stemmed from the finite-sample bias of MSM parameter estimation caused by outcome data sparsity at later trial visits among the always-treated when treatment prevalence was low, and among the never-treated when treatment prevalence was high. The outcome data sparsity in either treatment arm was further aggravated when increasing confounding strength. This was demonstrated in the data tabulation example in Table 1 of the Supplementary Materials.}
 

\begin{sidewaysfigure}[h!]
 \centering
 \includegraphics[width = \textwidth]{figures/New simulation figures/bias_surv0.jpeg}
 \caption{Empirical biases of the counterfactual survival probability estimator in the never-treated, $\wdiehat Pr(Y^{\bar 0}_{m,k} = 0)$, in various simulation scenarios.}
 \label{bias-0}
\end{sidewaysfigure}

\begin{sidewaysfigure}[h!]
 \centering
 \includegraphics[width = \textwidth]{figures/New simulation figures/bias_surv1.jpeg}
 \caption{Empirical biases of the survival probability estimates in the always-treated, $\wdiehat Pr(Y^{\bar 1}_{m,k} = 0)$, in various simulation scenarios.}
 \label{bias-1}
\end{sidewaysfigure}

\hl{Increasing the event rate tended to reduce absolute bias as the data sparsity issue was less severe. In high event rate scenarios, we observed positive bias in MRD estimation when treatment prevalence was high, due to overestimation of the  survival probability in the never-treated. This might be because,  with higher event rate and high treatment prevalence, outcome data sparsity mainly existed among the never-treated group, 
%thus   more likely to observe high-risk patients in the always-treated group, 
therefore overestimating the survival probability in the never-treated.
}

The empirical SD and the root-Mean Squared Error (MSE)  of the MRD estimates largely followed the patterns of the bias (see Figures 7 and 8 of the Supplementary Materials): scenarios with larger biases also exhibited larger SDs and MSEs. 

\subsubsection{Ratio of estimated standard errors to the empirical standard deviation of the MRD estimator}


Figures~\ref{fig:se_ratio_low} and \ref{fig:se_ratio_low_jackknifeMVN}\hl{present the summary statistics of the  SE ratios  for  each CI method, $\frac{\widehat{\rm SE}}{{\rm SD}_{\widehat{\rm MRD}}}$, in  scenarios with low event rates and small sample size ($n=200$); see Figures 9--13 of the Supplementary Materials for results in moderate and large sample sizes and low event rate scenarios, and the medium and high event rate scenarios.}

With small sample sizes, the SE ratios for nonparametric bootstrap CIs were on average lower than 1  at all visits,  and they were more variable at later visits and in  high treatment prevalence scenarios. 
This is consistent with the coverage results in Section~\ref{CIresults}, where we  expect nonparametric bootstrap CIs to have poor coverage if the variability of the MRD estimator was underestimated and the variability estimates were highly variable across simulations \cite{morris_using_2019}. 
The SE ratios for  jackknife Wald CIs were also lower than 1 at later visits, but in low and high treatment  prevalence scenarios, they were less variable compared to those for nonparametric bootstrap CIs, which might partly explain the better coverage of jackknife Wald CIs in these scenarios.  
However, the SE ratios for jackknife MVN CIs were much larger than 1 in  all scenarios with small sample sizes, which may explain the over-coverage for jackknife MVN CIs in some scenarios.

The SE ratios for LEF bootstrap CIs and Sandwich CIs were larger than 1 at early visits ($k<2$), but they gradually dropped below 1 at later visits, indicating underestimation of MRD estimation variability.    

When the treatment prevalence was high ($\alpha_a = 1$), their SE ratios were much lower but less variable than those for nonparametric bootstrap CIs at the later visits. 
In these small sample size scenarios, the better coverage of LEF bootstrap CIs  than nonparametric bootstrap CIs  might be partly attributed to  their overestimation of MRD estimation variability at early visits  and their less variable standard error estimates at later visits. 


\hl{With medium and large sample sizes ($n = 1000, 5000$) (Figure XXX of the Supplementary Materials)},  the LEF bootstrap CIs and Sandwich CIs tended to overestimate the empirical SD of the MRD, with their SE ratios being above 1 at most visits, which could explain some of the CI over-coverage we observed. The increase of sample size also reduced underestimation or overestimation of the empirical SD for all CI methods, as the SE ratios approaching 1 as sample sizes increased, while the same was observed when increasing outcome event rates. This is consistent with the coverage results in Section~\ref{CIresults}, where an increase of sample size and outcome event rate resulted in the various CI  methods converging to similar closer-to-nominal coverage. However, in scenarios with large sample sizes and low or high treatment prevalence, we still observed SE ratios to be lower than 1 and highly variable at later visits, which could explain the low coverage at later visits for all CI methods  in  these scenarios.

Similarly to the empirical coverage results, with other factors fixed, the confounding strength appeared to have minimal impact on sampling variability estimation shown by the SE ratios.


\begin{figure}[h]
 \centering
 \includegraphics[width = \textwidth]{figures/New simulation figures/mrd_se_low_200.jpeg}
 \caption{Ratio of the estimated standard error to empirical standard deviation of the MRD estimator under low event rates and small sample sizes. The dots represent the averages of the ratio,  with the bottom and top of the bar being the 1st and 3rd quartile of this ratio respectively. Bootstrap: CIs constructed by nonparametric bootstrap; LEF both: CIs constructed by applying Approach 2 of LEF bootstrap; LEF outcome: CIs constructed by applying Approach 1 of LEF bootstrap; Jackknife Wald: CIs constructed by applying Approach 1 of jackknife resampling; Sandwich: CIs based on the sandwich variance estimator. }
 \label{fig:se_ratio_low}
\end{figure}

\begin{figure}[h]
 \centering
 \includegraphics[width = \textwidth]{figures/New simulation figures/SE_ratio_jackknifeMVN_low.jpeg}
 \caption{Ratio of the estimated standard error to empirical standard deviation of the MRD estimator under low event rates and small sample sizes. The dots represent the averages of the ratio,  with the bottom and top of the bar being the 1st and 3rd quartile of this ratio respectively. Jackknife MVN: CIs constructed by applying Approach 2 of jackknife resampling.}
 \label{fig:se_ratio_low_jackknifeMVN}
\end{figure}

